Triplets of Mutually Unbiased Bases

We initiate a systematic study of triplets of mutually unbiased bases (MUBs). We show that in $\mathbb{C}^d$ each MUB-triplet is characterized by a $d\times d\times d$ object that we call a Hadamard cube. We describe the basic properties of Hadamard cubes, and show how an MUB-triplet can be reconstructed from such a cube, up to unitary equivalence. We also present an algebraic identity which is conjectured to hold for all MUB-triplets in dimension 6. If true, it would imply the long-standing conjecture of Zauner that the maximum number of MUBs in dimension 6 is three.

==> abbr.tex <==
\newcommand{\stb}{,\ldots,}
\newcommand{\then}{\Rightarrow}
\makeatletter
%GENERAL ALGEBRA
\newcommand{\subs}{\operatorname{subs}}
\newcommand{\ev}{\operatorname{even}}
%COMMUTATIVE ALGEBRA
\newcommand{\Ann}{\operatorname{Ann}}
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\Gg}{\operatorname{G}}
\newcommand{\Ff}{\operatorname{F}}
\newcommand{\Lie}{\operatorname{Lie}}
\newcommand{\Ee}{\operatorname{E}}
\renewcommand{\graph}{\operatorname{graph}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\Diff}{\operatorname{Diff}}
\renewcommand{\mod}{\operatorname{mod}}
\newcommand*\cat[1]{\mathbf{#1}}
%LINEAR ALGEBRA
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\Sp}{\operatorname{Sp}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\U}{\operatorname{U}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Ad}{\operatorname{Ad}}
\newcommand{\Fl}{\operatorname{Fl}}
\newcommand{\fd}{\operatorname{fd}}
\newcommand{\adim}{\operatorname{dim}^{\operatorname{alg}}}
\newcommand{\Fix}{\operatorname{Fix}}
\newcommand{\onto}{\twoheadrightarrow}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\Sch}{\overset{\circ}{\si}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\liminv}{\lim \operatorname{inv}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\Rep}{\operatorname{Rep}}
\newcommand{\rk}{\operatorname{rk}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\iso}{\cong}
\newcommand{\isoto}{\xrightarrow{\iso}}
\newcommand{\Inj}{\operatorname{Inj}}
\newcommand{\I}{I}
\newcommand{\J}{J}
%\newcommand{\K}{K}
\newcommand{\sii}{\boldsymbol \si}
\newcommand{\Omm}{\boldsymbol \Om}
\newcommand{\semi}{\rtimes}
\newcommand{\Irr}{\operatorname{Irr}}
\newcommand{\im}{\operatorname{Im}}
\newcommand{\acsa}{\qquad \iff\qquad}
\newcommand{\id}{\operatorname{id}}
\newcommand{\OSP}{\operatorname{OSP}}
\newcommand{\bra}{\langle}
\newcommand{\braaa}{[\![}
\newcommand{\ket}{\rangle}
\newcommand{\kettt}{]\!]}
\newcommand*\conj[1]{\overline{#1}}
%ANALYSIS
\newcommand{\res}{\operatorname{res}}
\renewcommand{\Re}{\operatorname{Re}}
\newcommand{\dd}{\,\mathrm{d}}
%GENERAL TOPOLOGY
\newcommand*\clos[1]{\overline{#1}}
\newcommand*\itemph[1]{\textbf{#1}}
\newcommand{\ZSq}{\operatorname{\Q Sq}}
%ALGEBRAIC TOPOLOGY
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\sing}{\operatorname{Sing}}
\newcommand{\Th}{\operatorname{Th}}
\newcommand{\Sq}{\operatorname{Sq}}
%\newcommand{\codim}{\operatorname{codim}}
\newcommand{\inj}{\hookrightarrow}
\newcommand{\RP}{\mathbb{R}P}
\newcommand{\CP}{\mathbb{C}P}
\newcommand{\HP}{\mathbb{H}P}
\newcommand{\OP}{\mathbb{O}P}
\renewcommand{\O}{\mathbb{O}}
\newcommand{\OO}{\mathcal{O}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\Gr}{\operatorname{Gr}}
\newcommand{\Pol}{\operatorname{Pol}}
\newcommand{\Sym}{\operatorname{Sym}}
%GREEK LETTERS
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\De}{\Delta}
\newcommand{\de}{\delta}
\newcommand{\ep}{\varepsilon}
\newcommand{\io}{\iota}
\newcommand{\ka}{\kappa}
\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\si}{\sigma}
\newcommand{\Si}{\Sigma}
\newcommand{\Om}{\Omega}
\newcommand{\om}{\omega}
%GROUP ACTIONS
\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\acts}{\curvearrowright}
\newcommand{\acted}{\curvearrowleft}
%SET OPERATIONS
\newcommand{\incl}{\hookrightarrow}
\newcommand{\se}{\subseteq}
\newcommand{\su}{\backslash}
\newcommand{\inter}{\operatorname{int}}
\newcommand{\Int}{\operatorname{Int}}
\newcommand{\chara}{\operatorname{char}}
%NUMBERS (R,C,Q...)
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\F}{\mathbb{F}}
%CALS
\newcommand{\T}{\mathcal{T}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\A}{\mathcal{A}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\VV}{\mathcal{V}}
%FRAKS
\renewcommand{\aa}{\mathfrak{a}}
\renewcommand{\sl}{\mathfrak{s}\mathfrak{l}}
\newcommand{\mm}{\mathfrak{m}}
\newcommand{\Spin}{\operatorname{Spin}}
\newcommand{\so}{\mathfrak{s}\mathfrak{o}}
\newcommand{\bb}{\mathfrak{b}}
\newcommand{\frakR}{\mathfrak{R}}
\newcommand{\kk}{\mathfrak{k}}
\newcommand{\q}{\mathfrak{q}}
\newcommand{\pp}{\mathfrak{p}}
\newcommand{\s}{\mathfrak{s}}
\newcommand{\frakt}{\mathfrak{t}}
\renewcommand{\gg}{\mathfrak{g}}
\newcommand{\ee}{\mathfrak{e}}
\newcommand{\ff}{\mathfrak{f}}
\newcommand{\uu}{\mathfrak{u}}
\newcommand{\hh}{\mathfrak{h}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\p}{\mathfrak{p}}
\newcommand{\git}{\mathbin{/\mkern-6mu/}}
\newcommand{\K}{\mathcal{K}}
%CATEGORIES
\newcommand{\TOP}{\mathrm{TOP}}
\newcommand{\SET}{\mathrm{SET}}
\newcommand{\hot}{\mathrm{hot}}
\newcommand{\cw}{\mathrm{CW}}
\newcommand{\CW}{\mathrm{CW}}
\newcommand{\alg}{\mathrm{ALG}}
\newcommand{\ab}{\Z-\mathrm{MOD}}
